Spatially dependent parton distribution functions and hard processes in nuclear collisions

This work focuses on applications of perturbative QCD (pQCD) and collinear factorization theorem to hard particle production in nuclear and hadronic collisions at the BNL-RHIC and CERN-LHC colliders. The emphasis is on nuclear parton distribution functions (nPDFs) and their spatial dependence. Also parton-to-hadron fragmentation functions (FFs) are studied. A brief overview of the applied theoretical and numerical tools is given in the introductory part.

==> hadlib_old.tex <==
\texttt{
LVW =(-2*N**4*(V-1)*VC*(V**5*W**5-5*V**4*W**4+10*V**3*W**3
  -10*V**2*W**2+5*V*W-1)*(V**5*W**5-5*(V-1)*V**4*W**4+10*(
  V-1)**2*V**3*W**3-10*(V-1)**3*V**2*W**2+5*(V-1)**4*V*W-(
  V-1)**5)*(16*V**5*W**5-16*V**4*(V+1)*W**4+V**3*(32*V**2-
  43*V+43)*W**3-V**2*(10*V**2-7*V+13)*W**2-(6*V**4-21*V**3
  +12*V**2+3*V-4)*W-4*(V-1)*(2*V**2-2*V+1))+2*N**2*(V-1)*V
  C*(V**3*(V+7)*W**3-V**2*(2*V**2+V+5)*W**2+(2*V**4+V**3-V
  +2)*W-4*(V-1)*(2*V**2-2*V+1))*(V**5*W**5-5*V**4*W**4+10*
  V**3*W**3-10*V**2*W**2+5*V*W-1)*(V**5*W**5-5*(V-1)*V**4*
  W**4+10*(V-1)**2*V**3*W**3-10*(V-1)**3*V**2*W**2+5*(V-1)
  **4*V*W-(V-1)**5)-2*(V-1)**2*VC*W*(V**3*W**2-2*V**3*W+(2
  *V-1)*(V**2-V+2))*(V**5*W**5-5*V**4*W**4+10*V**3*W**3-10
  *V**2*W**2+5*V*W-1)*(V**5*W**5-5*(V-1)*V**4*W**4+10*(V-1
  )**2*V**3*W**3-10*(V-1)**3*V**2*W**2+5*(V-1)**4*V*W-(V-1
  )**5))*LOG(1-V*W)/(N**2*(V-1)**3*V**2*W**2*(V*W-1)**5*(
  V*W-V+1)**5)}


==> hadlib_old_ex.tex <==

      LVW = (-2*N**4*(V-1)*VC*(V**5*W**5-5*V**4*W**4+10*V**3*W**3
     1   -10*V**2*W**2+5*V*W-1)*(V**5*W**5-5*(V-1)*V**4*W**4+10*(
     2   V-1)**2*V**3*W**3-10*(V-1)**3*V**2*W**2+5*(V-1)**4*V*W-(
     3   V-1)**5)*(16*V**5*W**5-16*V**4*(V+1)*W**4+V**3*(32*V**2-
     4   43*V+43)*W**3-V**2*(10*V**2-7*V+13)*W**2-(6*V**4-21*V**3
     5   +12*V**2+3*V-4)*W-4*(V-1)*(2*V**2-2*V+1))+2*N**2*(V-1)*V
     6   C*(V**3*(V+7)*W**3-V**2*(2*V**2+V+5)*W**2+(2*V**4+V**3-V
     7   +2)*W-4*(V-1)*(2*V**2-2*V+1))*(V**5*W**5-5*V**4*W**4+10*
     8   V**3*W**3-10*V**2*W**2+5*V*W-1)*(V**5*W**5-5*(V-1)*V**4*
     9   W**4+10*(V-1)**2*V**3*W**3-10*(V-1)**3*V**2*W**2+5*(V-1)
     :   **4*V*W-(V-1)**5)-2*(V-1)**2*VC*W*(V**3*W**2-2*V**3*W+(2
     ;   *V-1)*(V**2-V+2))*(V**5*W**5-5*V**4*W**4+10*V**3*W**3-10
     <   *V**2*W**2+5*V*W-1)*(V**5*W**5-5*(V-1)*V**4*W**4+10*(V-1
     =   )**2*V**3*W**3-10*(V-1)**3*V**2*W**2+5*(V-1)**4*V*W-(V-1
     >   )**5))*LOG(1-V*W)/(N**2*(V-1)**3*V**2*W**2*(V*W-1)**5*(
     ?   V*W-V+1)**5)


